A Game Theoretic Macroscopic Model of Bypassing at Traffic Diverges with Applications to Mixed Autonomy Networks

Vehicle bypassing is known to negatively affect delays at traffic diverges. However, due to the complexities of this phenomenon, accurate and yet simple models of such lane change maneuvers are hard to develop. In this work, we present a macroscopic model for predicting the number of vehicles that bypass at a traffic diverge. We take into account the selfishness of vehicles in selecting their lanes; every vehicle selects lanes such that its own cost is minimized. We discuss how we model the costs experienced by the vehicles. Then, taking into account the selfish behavior of the vehicles, we model the lane choice of vehicles at a traffic diverge as a Wardrop equilibrium. We state and prove the properties of Wardrop equilibrium in our model. We show that there always exists an equilibrium for our model. Moreover, unlike most nonlinear asymmetrical routing games, we prove that the equilibrium is unique under mild assumptions. We discuss how our model can be easily calibrated by running a simple optimization problem. Using our calibrated model, we validate it through simulation studies and demonstrate that our model successfully predicts the aggregate lane change maneuvers that are performed by vehicles for bypassing at a traffic diverge. We further discuss how our model can be employed to obtain the optimal lane choice behavior of the vehicles, where the social or total cost of vehicles is minimized. Finally, we demonstrate how our model can be utilized in scenarios where a central authority can dictate the lane choice and trajectory of certain vehicles so as to increase the overall vehicle mobility at a traffic diverge. Examples of such scenarios include the case when both human driven and autonomous vehicles coexist in the network. We show how certain decisions of the central authority can affect the total delays in such scenarios via an example.

==> uniqueness.tex <==
\section{Prior Work }\label{sec:uniq}
\begin{figure}
\centering
\begin{tikzpicture}[scale=1.2]
\begin{scope}[every node/.style={circle,thick,draw}]
    \node (A) at (0,0) {A};
    \node (B) at (3,1.5) {B};
    \node (C) at (3,-1.5) {C};
    \node (D) at (6,0) {D};
    
\end{scope}

\begin{scope}[>={Stealth[teal]},
              every node/.style={fill=white,circle},
              every edge/.style={draw=teal,very thick}]
    \path [->] (A) edge node {$1$} (B);
    \path [->] (A) edge node {$3$} (C);
    \path [->] (B) edge node {$2$} (D);
    \path [->] (C) edge node {$4$} (D);
   %\path [->] (A) edge node {$4$} (D);
    %\path [->] (D) edge node {$3$} (C);
    %\path [->] (A) edge node {$3$} (E);
    %\path [->] (D) edge node {$3$} (E);
    %\path [->] (D) edge node {$3$} (F);
    %\path [->] (C) edge node {$5$} (F);
    %\path [->] (E) edge node {$8$} (F); 
    %\path [->] (B) edge[bend right=60] node {$1$} (E); 
\end{scope}

\end{tikzpicture}
\caption{A network with a single O/D pair and two paths.}\label{fig:net_equ}
\end{figure}

%Knowing that the network always has an equilibrium, we need to study the uniqueness of the equilibrium. 
\subsection{Existence of Equilibrium}
We state the following proposition from~\cite{braess1979existence}
which studies the conditions under which the Wardrop Equilibrium exists for a multiclass traffic network.
%A natural question that can be raised in the setting of networks with mixed autonomy is whether there exists an equilibrium. Noting that our game is an instance of multi class routing games, recall the following from~\cite{braess1979existence}.

\begin{proposition}\label{prop:exist}
Given a network $G = (N,L,W)$, if the link delay functions are continuous and monotone in the link flow of each class; then, there exists at least one Wardrop equilibrium. 
%along with nonnegative, continuous and nondecreasing link latency functions $e_l$, there exists at least one equilibrium for the game. 
\end{proposition}

%\noindent As mentioned previously, for a given profile of $\alpha_w$'s, each type of vehicles, regular or autonomous, can be modeled as a separate commodity. 
\begin{remark}
\label{remark:exist}
Using~\eqref{eq:latency_simplified}, since our assumed delay functions are nonnegative, continuous, and monotone in the flow of each class, Proposition~\ref{prop:exist} implies that there always exists at least one Wardrop equilibrium for a routing game with mixed autonomy. 
\end{remark}



\subsection{Uniqueness of Equilibrium}
In this part, we review the known results regarding the uniqueness of Wardrop Equilibrium. When multiple classes of vehicles are present in the network, the uniqueness of the equilibrium flow vector does not hold. However, uniqueness in a weak sense is known to hold from~\cite{altman2006survey}.

%The followings are known about the uniqueness of Wardrop equilibrium from~\cite{altman2002competitive} and~\cite{altman2006survey}, respectively:

%\begin{proposition}
%\label{prop:strong_uniq}
%For a general topology network $G$ with only one class of vehicles on each O/D pair, along with delay functions of the form~\eqref{eq:latency_func}, the equilibrium flow vector $f$ is unique. 
%\end{proposition}
%
 
\begin{proposition}\label{prop:weak_uniq}For a general topology network $G$ with multiple classes of vehicles on each O/D pair, if the delay functions are of the form~\eqref{eq:latency_func}, and the link capacities $C_l$ are fixed and the same for all vehicle classes, for a given demand vector $r$, we have

\begin{enumerate}
\item The equilibrium is unique in a weak sense, i.e. for each link $l$ the total flow $f_l$ is unique. 
\item For each O/D pair $w \in W$, the delay of travel $e_w(f)$ is unique for all Wardrop equilibrium flow vectors $f$. Thus, the delay of travel for each O/D pair $e_w(f)$ is a well defined function of network demand vector $r$ and can be rewritten as $e_w(r)$.
\end{enumerate} 
\end{proposition}

\begin{remark}\label{rem:sing_type}
Note that a routing game that has only a single class of vehicles can be viewed as an instance of the games described in Proposition~\ref{prop:weak_uniq}. Therefore, uniqueness in a the weak sense applies to games with a single type of vehicles too. 
\end{remark}
%If there exists a single commodity of vehicles, under the assumption of BPR latency function~\eqref{eq:latency_func}, the flow vector $\f$ was proved to be unique in~\cite{altman2002competitive}. When there are multiple commodities of flows in the network, Wardrop equilibrium is known to be unique in a weak sense: the total flow on each link is unique rather than the flow of each commodity on a link~\cite{altman2006survey}. 


\subsection{Monotonicity of Social Delay}


As we discussed above, in general, the equilibrium is not unique. However, if the conditions of Proposition~\ref{prop:weak_uniq} hold for a network, the social delay and the delay of travel for each O/D pair  are unique.
For a single class routing game on $G = (N, L, W)$, 
%with an abuse of notation,  we denote the delay of travel for an O/D pair $w \in W$ in the network by $e_w(r)$, where $r = (r_w: w \in W)$ is the demand profile of the network. 
%Aligned with this,
recall the following from~\cite{hall1978properties}.  
\begin{proposition}\label{prop:contin_latency}
Consider a network $G = (N,L,W)$, where only one class of vehicles exist for each O/D pair $w$. Assume that for  each link $l \in L$, $e_l(.)$ is continuous, positive valued, and monotonically increasing. Then, for each $w \in W$, the delay of travel $e_w(r)$ is a continuous function of the demand vector $r$. Furthermore, $e_w(.)$ is nonincreasing in $r_w$ when all other demands $r_{w'}, w' \neq w$, are fixed. 
\end{proposition}


 %Table summarizes the maximum and minimum path flows in the equilibria of the system. Clearly, the uniqueness does not hold even in the weak sense. 

%\begin{table}
%\begin{center}
%\begin{tabular}{ |l|l|l| }
%\hline
%\multicolumn{3}{ |c| }{Team sheet} \\
%\hline
% & Minimum Path Flow & Maximum Path Flow \\ \hline
%$f_{ABD}$ & 0.75 & 1.25 \\ \hline
%$f_{ACD}$ & 0.75 & 1.25 \\ \hline
%\end{tabular}.
%\end{center}
%\end{table}



